Class-Conditioned Transformation for Enhanced Robust Image Classification

Robust classification methods predominantly concentrate on algorithms that address a specific threat model, resulting in ineffective defenses against other threat models. Real-world applications are exposed to this vulnerability, as malicious attackers might exploit alternative threat models. In this work, we propose a novel test-time threat model agnostic algorithm that enhances Adversarial-Trained (AT) models. Our method operates through COnditional image transformation and DIstance-based Prediction (CODIP) and includes two main steps: First, we transform the input image into each dataset class, where the input image might be either clean or attacked. Next, we make a prediction based on the shortest transformed distance. The conditional transformation utilizes the perceptually aligned gradients property possessed by AT models and, as a result, eliminates the need for additional models or additional training. Moreover, it allows users to choose the desired balance between clean and robust accuracy without training. The proposed method achieves state-of-the-art results demonstrated through extensive experiments on various models, AT methods, datasets, and attack types. Notably, applying CODIP leads to substantial robust accuracy improvement of up to $+23\%$, $+20\%$, $+26\%$, and $+22\%$ on CIFAR10, CIFAR100, ImageNet and Flowers datasets, respectively.

==> tables/rebuttal_rs.tex <==

\begin{table}[h!]
\begin{center}
\caption{
    \textbf{Randomized Smoothing CIFAR-10}
    % \vspace{-30pt}
}
\resizebox{0.5\textwidth}{!}{%

\begin{tabular}{lccccc}
\hline\noalign{\smallskip}\hline

\rowcolor{gray!5} Method & Clean & $8/255$ & $16/255$ & $0.5$ & $1.0$\\
% \rowcolor{gray!5} & & \multicolumn{2}{c}{$L_{\infty}$} & \multicolumn{2}{c}{$L_{2}$}\\
% \rowcolor{gray!5} \multirow{-3}{*}{Method} & \multirow{-3}{*}{Clean} & $8/255$ & $16/255$ & $0.5$ & $1.0$\\

\hline\noalign{\smallskip}\hline\noalign{\smallskip}


\multirow{1}{*}{AT [29]} & $89.43\%$ &  $30.84\%$ & $01.23\%$ & $68.94\%$ & $38.53\%$\\




\hline\noalign{\smallskip} \hline\noalign{\smallskip}



\end{tabular}%
}
\vspace{-20pt}
\label{table:reb_rs}
\end{center}
\end{table}


==> tables/rebuttal_top_k_attack.tex <==

\begin{table}[h!]
\vspace{-10pt}
\begin{center}
\caption{
    \textbf{Top-k Attack Analysis CIFAR-100} 
}
\resizebox{\columnwidth}{!}{%

\begin{tabular}{llcccc}
\hline\noalign{\smallskip}\hline

\rowcolor{gray!5}  &  & \multicolumn{3}{c}{Top-k} \\
\rowcolor{gray!5} \multirow{-2}{*}{Method} & \multirow{-2}{*}{Attack}  & 1 & 20 & 40 \\

\multirow{2}{*}{Rebuffi et al. [35]} & TPO & $61.71\%$ & $95.43\%$ & $98.43\%$ \\
 & TPIO & $38.56\%$ & $84.20\%$ & $92.62\%$ \\



% \hline\noalign{\smallskip}

% \multirow{2}{*}{Gowal et al. [17]} & TPO & $61.65\%$ & $95.50\%$ & $98.53\%$ \\
%  & TPIO & $43.73\%$ & $85.58\%$ & $93.40\%$ \\


\hline\noalign{\smallskip}\hline\noalign{\smallskip}


\end{tabular}

}


\label{table:reb_top_k}

\end{center}
\vspace{-20pt}
\end{table}





